Solving Parabolic Moving Interface Problems with Dynamical Immersed Spaces on Unfitted Meshes: Fully Discrete Analysis

Immersed finite element (IFE) methods are a group of long-existing numerical methods for solving interface problems on unfitted meshes. A core argument of the methods is to avoid mesh regeneration procedure when solving moving interface problems. Despite the various applications in moving interface problems, a complete theoretical study on the convergence behavior is still missing. This research is devoted to close the gap between numerical experiments and theory. We present the first fully discrete analysis including the stability and optimal error estimates for a backward Euler IFE method for solving parabolic moving interface problems. Numerical results are also presented to validate the analysis.

==> symbol.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}






%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

\usepackage{amsmath}
\usepackage[thmmarks,amsmath,amsthm]{ntheorem}
\usepackage{comment}

\usepackage{amsfonts, psfrag, graphicx, amssymb,enumitem,indentfirst,float,geometry,color,enumerate,graphicx,subcaption,algorithm,algpseudocode,pifont,hyperref,mathtools,gensymb}
%\usepackage{refcheck}
\usepackage{pbox}
\usepackage{booktabs, cellspace, hhline}
\setlength\cellspacetoplimit{4pt}
\setlength\cellspacebottomlimit{4pt}



\allowdisplaybreaks[4]
\geometry{left=1.9cm,right=1.9cm,top=1.9cm,bottom=1.9cm}
\renewcommand{\baselinestretch}{0.97}

\numberwithin{equation}{section}
\numberwithin{figure}{section}

%\usepackage{lipsum}
\usepackage{etoolbox}
\patchcmd{\thebibliography}{\chapter*}{\section*}{}{}
\usepackage[sectionbib]{natbib}
\usepackage[title]{appendix}

\usepackage{lipsum}
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\newtheorem{hyp}{Hypothesis}
%\newtheorem{algorithm}{Algorithm}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{thm}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{rem}{Remark}[section]
\newtheorem{asump}{Assumption}[section]

%\usepackage{chngcntr} %%%%%%%%%%%%%%%%%% in this latex version, this package is not necessary
\counterwithin{table}{section}

\newcommand{\commentout}[1]{{}} % for large block comments

%\newtheorem{thm}{Theorem}
%\newtheorem{rem}{Remark}
%\newtheorem{exmp}{Example}
%\newtheorem{lemma}{Lemma}
%\numberwithin{thm}{section}
%\numberwithin{exmp}{section}
%\numberwithin{lemma}{section}
%\numberwithin{rem}{section}

\newcommand{\Frac}[2]{\frac{\textstyle #1}{\textstyle #2}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\|#1\right\|}

\newcommand{\bfA}{{\bf A}}
\newcommand{\bfa}{{\bf a}}
\newcommand{\bfB}{{\bf B}}
\newcommand{\bfb}{{\bf b}}
\newcommand{\bfC}{{\bf C}}
\newcommand{\bfc}{{\bf c}}
\newcommand{\bfD}{{\bf D}}
\newcommand{\bfd}{{\bf d}}
\newcommand{\bfE}{{\bf E}}
\newcommand{\bfe}{{\bf e}}
\newcommand{\bfF}{{\bf F}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfG}{{\bf G}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfH}{{\bf H}}
\newcommand{\bfh}{{\bf h}}
\newcommand{\bfI}{{\bf I}}
\newcommand{\bfi}{{\bf i}}
\newcommand{\bfj}{{\bf j}}
\newcommand{\bfJ}{{\bf J}}
\newcommand{\bfk}{{\bf k}}
\newcommand{\bfK}{{\bf K}}
\newcommand{\bfl}{{\bf l}}
\newcommand{\bfL}{{\bf L}}
\newcommand{\bfM}{{\bf M}}
\newcommand{\bfm}{{\bf m}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bfN}{{\bf N}}
\newcommand{\bfP}{{\bf P}}
\newcommand{\bfp}{{\bf p}}
\newcommand{\bfQ}{{\bf Q}}
\newcommand{\bfq}{{\bf q}}
\newcommand{\bfR}{{\bf R}}
\newcommand{\bfr}{{\bf r}}
\newcommand{\bfs}{{\bf s}}
\newcommand{\bfS}{{\bf S}}
\newcommand{\bft}{{\bf t}}
\newcommand{\bfT}{{\bf T}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfV}{{\bf V}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfw}{{\bf w}}
\newcommand{\bfW}{{\bf W}}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfX}{{\bf X}}
\newcommand{\x}{{\bf x}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfY}{{\bf Y}}
\newcommand{\bfz}{{\bf z}}
\newcommand{\bfZ}{{\bf Z}}


\newcommand{\bfalpha}{{\boldsymbol \alpha}}
\newcommand{\bfbeta}{{\boldsymbol \beta}}
\newcommand{\bfdelta}{\boldsymbol{\delta}}
\newcommand{\bfepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bfgamma}{\boldsymbol{\gamma}}
\newcommand{\bfGamma}{\boldsymbol{\Gamma}}
\newcommand{\bfLambda}{\boldsymbol{\Lambda}}
\newcommand{\bfphi}{\boldsymbol{\phi}}
\newcommand{\bfPhi}{\boldsymbol{\Phi}}
\newcommand{\bfpsi}{\boldsymbol{\psi}}
\newcommand{\bfPsi}{\boldsymbol{\Psi}}
\newcommand{\bfsigma}{\boldsymbol{\sigma}}
\newcommand{\bftau}{\boldsymbol{\tau}}
\newcommand{\bftheta}{\boldsymbol{\theta}}
\newcommand{\bfTheta}{\boldsymbol{\Theta}}
\newcommand{\bfxi}{\boldsymbol{\xi}}
\newcommand{\bfzeta}{\boldsymbol{\zeta}}

\newcommand{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\verti}[1]{{\left\vert #1
    \right\vert}}
